Hand Trajectory Fusion for Egocentric Natural Language Query Grounding

Egocentric Natural Language Query (NLQ) grounding asks a model to localize, in a long first-person video, the temporal interval that answers a free-form text query. Existing methods fuse video appearance with the query but ignore hand motion, despite the fact that roughly 41% of Ego4D NLQ queries are answered at a moment of hand--object manipulation or their immediate outcomes. We propose a hand-trajectory encoder for converting a sequence of hand skeletons into highly-semantic hand kinematic features, which are then aligned and combined with pretrained video--text features through a cross-attention fusion strategy with adaptive gating. On the Ego4D NLQ v2 validation split, the clearest gains appear for Hand-Object Interaction queries (+2.54 R1@IoU=0.3) and Quantity/State queries (+4.32 R1@IoU=0.3), indicating that hand trajectory provides grounding cues beyond appearance alone.

==> sec/2_related.tex <==
% %--------------------------------------------------------------
% \section{Related Work}
% \label{sec:related}
% %--------------------------------------------------------------

% \paragraph{Natural Language Query grounding.}
% In recent years, this topic has received increasing attention. Moment-DETR~\cite{Lei2021MomentDETR} established the set-prediction paradigm for moment retrieval via learnable queries and Hungarian matching, which subsequent methods build upon.
% On Ego4D~\cite{Grauman2022}, NaQ~\cite{Ramakrishnan2023NaQ} introduced a data augmentation strategy using narration clips as weak supervision, substantially improving recall.
% GroundNLQ~\cite{GroundNLQ} proposed a two-stage pipeline: narration pre-training on EgoClip followed by NLQ fine-tuning, using a ConvTransformer backbone with cross-modal video-text attention.
% UniVTG~\cite{Lin2023UniVTG} unified moment retrieval, highlight detection, and video summarization through large-scale pre-training.
% R2-Tuning~\cite{R2Tuning} improved efficiency by selective temporal fine-tuning of image-pretrained representations.
% EgoVideo~\cite{Pei2024EgoVideo} adapted an egocentric foundation model to temporal grounding, showing that domain-specific pretraining scale is a primary driver of performance.
% Our work extends GroundNLQ by injecting hand trajectory as an auxiliary modality while keeping the pretrained video-text backbone frozen.

% \paragraph{Egocentric video features and pretraining.}
% Strong visual representations are the primary driver of NLQ performance.
% EgoVLP~\cite{Lin2022EgoVLP} established egocentric-specific contrastive pretraining (EgoNCE) on EgoClip, dramatically improving recall over general-purpose encoders.
% EgoVLPv2~\cite{Pramanick2023EgoVLPv2} extended this by performing video-language fusion inside the backbone rather than after it, achieving better cross-modal alignment with the same feature footprint.
% LaVILA~\cite{Zhao2023LaVILA} leverages large language models to generate dense video narrations as pretraining supervision, producing features now used by top NLQ systems~\cite{OSGNet}.
% InternVideo~\cite{Wang2022InternVideo} demonstrated that scale, generative and discriminative pretraining on broad video data, yields features competitive with domain-specific encoders.
% We follow GroundNLQ and concatenate InternVideo\allowbreak+\allowbreak EgoVLP features, keeping our gains orthogonal to backbone feature engineering.

% \paragraph{Auxiliary modality fusion for NLQ.}
% GazeNLQ~\cite{GazeNLQ} is the closest prior work: it adds predicted gaze as an auxiliary modality to GroundNLQ via a dedicated gaze encoder and sum-residual cross-attention, achieving state-of-the-art results on Ego4D NLQ.
% Gaze is a dense signal (a 1D scalar per frame, always available) with a simple spatial semantics.
% ObjectNLQ~\cite{Feng2024ObjectNLQ} introduced an object detection branch to augment video representations for NLQ, showing that spatially grounded auxiliary signals improve temporal localization; it is analogous to our work but targets object identity rather than hand kinematics.
% OSGNet~\cite{OSGNet}, the CVPR 2025 challenge winner, fuses video features with object detection features (CO-DETR) and LaVILA captions through early fusion inside the backbone; it also uses BiMamba temporal modeling and train+val data.
% In contrast, hand trajectory is a higher-dimensional, sparse signal (21 3D keypoints per frame, detected in only $\sim$41\% of frames) that encodes kinematic structure rather than visual attention or object identity.
% No published work has studied hand trajectory as an auxiliary modality for Ego4D NLQ grounding.

% \paragraph{Hand pose and trajectory encoding.}
% MediaPipe Hands~\cite{Zhang2020MediaPipe} provides 21 normalized 3D keypoints per hand in real time without GPU inference, and has been validated on egocentric video.
% Graph-based methods like ST-GCN~\cite{Yan2018STGCN} and MotionBERT~\cite{Zhu2023MotionBERT} model full-body pose sequences with spatio-temporal graph convolutions or transformer encoders.
% In the egocentric domain, Liu \etal~\cite{Liu2022HOIForecast} predict future hand trajectories and object contact hotspots from first-person video using an object-centric transformer; we instead use past hand trajectories as a temporal grounding signal rather than for forecasting.
% EgoHOD~\cite{Pei2025EgoHOD} models fine-grained hand-object dynamics as pretraining supervision for egocentric representations, providing evidence that kinematic signals carry task-relevant information complementary to appearance features.
% We adopt a factorized transformer design, spatial attention over the 21-landmark graph followed by temporal windowed attention, which is more parameter-efficient than graph convolutions and handles the variable-length, sparse input naturally through attention masking.

